Exact and Approximate Hierarchical Clustering Using A*

Hierarchical clustering is a critical task in numerous domains. Many approaches are based on heuristics and the properties of the resulting clusterings are studied post hoc. However, in several applications, there is a natural cost function that can be used to characterize the quality of the clustering. In those cases, hierarchical clustering can be seen as a combinatorial optimization problem. To that end, we introduce a new approach based on A* search. We overcome the prohibitively large search space by combining A* with a novel \emph{trellis} data structure. This combination results in an exact algorithm that scales beyond previous state of the art, from a search space with $10^{12}$ trees to $10^{15}$ trees, and an approximate algorithm that improves over baselines, even in enormous search spaces that contain more than $10^{1000}$ trees. We empirically demonstrate that our method achieves substantially higher quality results than baselines for a particle physics use case and other clustering benchmarks. We describe how our method provides significantly improved theoretical bounds on the time and space complexity of A* for clustering.

==> tex/alg_tree_astar.tex <==

\begin{algorithm}
 \label{alg:tree-astar-old}
 \caption{A* Hierarchical Clustering Search}
 \begin{algorithmic}
\Function{InitializeVertex}{$\trellis$, $\dataset_\ell$, $\Hfun$}
    %\tree_\maxsplit(\dataset)
    %\State $\trellis[\dataset_\ell]$.MAP\_value = $Null$
    \State $\tree^{*}_\maxsplit(\dataset)$ = $Null$
    \State $\dataset_\ell[\frontier] = $ get\_children$(\trellis, \dataset_\ell$)
    \State heapify$(\dataset_\ell[\frontier], \Hfun)$
    \State $g, h, \dataset_L, \dataset_R  = \dataset_\ell[\frontier]$.peek()
    \State \textbf{return} $g, h$
\EndFunction
\Function{ExecuteSearch}{$\trellis$, $\dataset_\ell$, $\Hfun$}
%    \If{$\trellis[\dataset_\ell]$.MAP\_value $\neq Null$}
    \If{$\tree^{*}_\maxsplit(\dataset) \neq Null$}
    \State \textbf{return} $\tree^{*}_\maxsplit(\dataset), 0$
    \EndIf
    \If{not is\_explored($\dataset_\ell$)}
      \State \textbf{return} \Call{InitializeVertex}{$\trellis$, $\dataset_\ell$, $\Hfun$}
    \EndIf
    \State $g, h, \trellisVertex_L, \trellisVertex_R  = \dataset_\ell[\frontier]$.dequeue()
    \If{h = 0}
        \State $\tree^{*}_\maxsplit(\dataset) = g$
    \Else
        \State $g_L, h_L =$ \Call{ExecuteSearch}{$\trellis[\dataset_L]$,  $ \dataset_L$, $\Hfun$}
        \State $g_R, h_R =$ \Call{ExecuteSearch}{$\trellis[\dataset_R]$,  $\dataset_R$, $\Hfun$}
        \State $g = \EfunS(\dataset_L, \dataset_R) + g_L + g_R$
        \State $h = h_L + h_R$
    \EndIf
    \State $\dataset_\ell[\frontier]$.enqueue($g, h, \dataset_L, \dataset_R$)
    \State $g, h, \dataset_L, \dataset_R  = \dataset_\ell[\frontier]$.peek()
    \State \textbf{return} $g, h$
\EndFunction
\Function{A*TreeMAPSearch}{$\trellis$, $\dataset$, $\Hfun$}
   \While{$h \neq 0$}
   \State $g, h =$ \Call{ExecuteSearch}{$\trellis$, $\dataset$, $\Hfun$}
   \EndWhile
\EndFunction
  \end{algorithmic}
\end{algorithm}


